In-The-Field Monitoring of Functional Calls: Is It Feasible?

Collecting data about the sequences of function calls executed by an application while running in the field can be useful to a number of applications, including failure reproduction, profiling, and debugging. Unfortunately, collecting data from the field may introduce annoying slowdowns that negatively affect the quality of the user experience. So far, the impact of monitoring has been mainly studied in terms of the overhead that it may introduce in the monitored applications, rather than considering if the introduced overhead can be really recognized by users. In this paper we take a different perspective studying to what extent collecting data about sequences of function calls may impact the quality of the user experience, producing recognizable effects. Interestingly we found that, depending on the nature of the executed operation and its execution context, users may tolerate a non-trivial overhead. This information can be potentially exploited to collect significant amount of data without annoying users.

==> tables/adobe_reader.tex <==
% !TEX root =  ../NIER_Extension.tex

%\begin{table}[h]
%\centering
%\scriptsize
%\begin{tabular}{lc|ccccccc}
%\hline
%\multicolumn{2}{l|}{}                        & \multicolumn{6}{c}{With Monitoring}                                                                                                                                                                                 &                                                        \\ \hline
%Action Category & \multicolumn{1}{l|}{Total} & \multicolumn{1}{l}{Inst.} & \multicolumn{1}{l}{Imm.} & \multicolumn{1}{l}{Cont. Simple} & \multicolumn{1}{l}{Cont. Complex} & \multicolumn{1}{l}{Capt.} & \begin{tabular}[c]{@{}c@{}}$>$ Cap.\end{tabular} & \begin{tabular}[c]{@{}c@{}}\%Slow\\Actions\end{tabular} \\ \hline
%Instantaneous   & 55                        & 50                        & 5                        & 0                                & 0                                 & 0                         & 0                                                         & 9                                                      \\ \hline
%Immediate       & 15                        & 0                         & 15                       & 0                                & 0                                 & 0                         & 0                                                         & 0                                                      \\ \hline
%Cont. Simple    & 90                        & 0                         & 0                        & 69                               & 16                                & 5                         & 0                                                         & 23                                                     \\ \hline
%Cont. Complex   & 15                        & 0                         & 0                        & 0                                & 13                                & 1                         & 1                                                         & 13                                                      \\ \hline
%Captive         & 0                         & 0                         & 0                        & 0                                & 0                                 & 0                         & 0                                                         & 0                                                      \\ \hline
%\end{tabular}
%\caption{Adobe Acrobat Reader DC: actions classification in the control execution and in the monitoring executions}
%\label{adobeSA}
%\end{table}


\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lc|ccccccc}
        \toprule
%\multicolumn{2}{l|}{}                        & \multicolumn{6}{c}{With Monitoring}                                                                                                                                                                                 &                                                        
	 \begin{tabular}{c} \textbf{Action} \\ \textbf{Category} \end{tabular} 
	 & \textbf{Total}
	& \textbf{Instantaneous}
	& \textbf{Immediate}
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Simple} \end{tabular} 
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Complex} \end{tabular} 
	& \textbf{Captive}
	& $>$ \textbf{Captive}	
	& \begin{tabular}[c]{@{}c@{}} \textbf{Slow}\\\textbf{Actions [\%]}\end{tabular} \\ 
	 \midrule
	Instantaneous	& 55	& \cellcolor{lightgray}50	& \textbf{5}	& 0	& 0	& 0	& 0	& \textbf{9\%} \\ \midrule
	Immediate       & 15                        & 0                         & \cellcolor{lightgray}15                       & 0                                & 0                                 & 0                         & 0                                                         & \textbf{0\%}                                                      \\   \midrule
Continuous Simple    & 90                        & 0                         & 0                        & \cellcolor{lightgray}69                               &  \textbf{16}                                &  \textbf{5}                         & 0                                                         &  \textbf{23\%}                                                     \\   \midrule
Continuous Complex   & 15                        & 0                         & 0                        & 0                                & \cellcolor{lightgray}13                                &  \textbf{1}                         &  \textbf{1}                                                         &  \textbf{13\%}                                                      \\   \midrule
Captive         & 0                         & 0                         & 0                        & 0                                & 0                                 & \cellcolor{lightgray}0                         & 0                                                         &  \textbf{0\%}                                                      \\  
      \bottomrule
\end{tabular}
}
%\caption{Adobe Acrobat Reader DC: actions classification in the control execution and in the monitoring executions}
\caption{Adobe Reader DC: distribution of the typologies of actions with and without probe}
\label{table-adobeSA}
\end{table}

==> tables/cpu60.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lccc|ccc}
        \toprule

 \multirow{2}[2]{*}{ \textbf{SRT Category}}  & \multicolumn{3}{c}{\textbf{Overhead}} & \multicolumn{3}{c}{\textbf{Slow actions}} \\  \cmidrule{2-7}
& \textbf{CPU only}  & \textbf{CPU \& Monitoring}  & \textbf{$\Delta$} & \textbf{CPU only}  & \textbf{CPU \& Monitoring}  & \textbf{$\Delta$}\\   \midrule

%\textbf{CPU 60\% {[}\%{]}} & \textbf{Slow Actions {[}\%{]}} & Monitoring {[}\%{]} & Slow Actions {[}\%{]} & $\Delta$ Overhead {[}\%{]} & $\Delta$ Slow Actions {[}\%{]} \\  \midrule
%Instantaneous & 5.85              & 40.61                 & 9.72                     & 57.58                 & 3.87                    & 16.97                       \\ \midrule
Instantaneous & 5.85           & 9.72   & 3.87   & 40.61                                 & 57.58                                   & 16.97                       \\ \midrule
%Immediate     & 6.64              & 13.33                 & 44.76                    & 36.67                 & 38.12                   & 23.33                       \\ \midrule
Immediate     & 6.64              & 44.76   & 38.12     & 13.33                         & 36.67                               & 23.33                       \\ \midrule
%Continuous Simple  & 4.48              & 8.24                  & 93.65                    & 30.29                 & 89.17                   & 22.06                       \\ \midrule
Continuous Simple  & 4.48          & 93.65         & 89.17   & 8.24                                  & 30.29                                 & 22.06                       \\ \midrule
%Continuous Complex & 19.31             & 32.22                 & 108.54                   & 66.67                 & 89.23                   & 34.44                       \\ \midrule
Continuous Complex & 19.31            & 108.54   & 89.23   & 32.22                                   & 66.67                                  & 34.44                       \\ \midrule
%Captive       & 93.58             & 16.67                 & 144.57                   & 21.67                 & 51.00                   & 5.00                        \\ 
Captive       & 93.58            & 144.57  & 51.00 & 16.67                                    & 21.67                                    & 5.00                        \\ 
\bottomrule
\end{tabular}
}
\caption{Overhead impact of CPU load 60\%}
\label{table:cpu60}
\end{table}

==> tables/cpu60_old.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{l|cc|cc|cc|}
        \toprule


\textbf{SRT Category}  & \textbf{CPU 60\% {[}\%{]}} & \textbf{Slow Actions {[}\%{]}} & Monitoring {[}\%{]} & Slow Actions {[}\%{]} & $\Delta$ Overhead {[}\%{]} & $\Delta$ Slow Actions {[}\%{]} \\  \midrule
Instantaneous & 5.85              & 40.61                 & 9.72                     & 57.58                 & 3.87                    & 16.97                       \\ \midrule
Immediate     & 6.64              & 13.33                 & 44.76                    & 36.67                 & 38.12                   & 23.33                       \\ \midrule
Continuous Simple  & 4.48              & 8.24                  & 93.65                    & 30.29                 & 89.17                   & 22.06                       \\ \midrule
Continuous Complex & 19.31             & 32.22                 & 108.54                   & 66.67                 & 89.23                   & 34.44                       \\ \midrule
Captive       & 93.58             & 16.67                 & 144.57                   & 21.67                 & 51.00                   & 5.00                        \\ 
\bottomrule
\end{tabular}
}
\caption{Overhead impact of CPU load 60\%}
\label{table:cpu60}
\end{table}

==> tables/cpu75.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lccc|ccc}
        \toprule

 \multirow{2}[2]{*}{ \textbf{SRT Category}}  & \multicolumn{3}{c}{\textbf{Overhead}} & \multicolumn{3}{c}{\textbf{Slow actions}} \\  \cmidrule{2-7}
& \textbf{CPU only}  & \textbf{CPU \& Monitoring}  & \textbf{$\Delta$} & \textbf{CPU only}  & \textbf{CPU \& Monitoring}  & \textbf{$\Delta$}\\   \midrule


%SRT Category  & CPU 75\% {[}\%{]} & Slow Actions {[}\%{]} & Monitoring {[}\%{]} & Slow Actions {[}\%{]} & $\Delta$ Overhead {[}\%{]} & $\Delta$ Slow Actions {[}\%{]} \\ \hline
Instantaneous 		& 8.04              & 13.55  & 5.51      & 70.30                            & 75.76                   & 5.46                                     \\ \midrule
Immediate     		& 18.39           & 44.71      & 26.32      & 26.67                              & 53.33                              & 26.67                       \\ \midrule
Continuous Simple  	& 17.86           & 100.76      & 82.90      & 17.94                           & 30.59                              & 12.65                       \\ \midrule
Continuous Complex & 38.81           & 172.58        & 133.78     & 37.78                       & 73.33                          & 35.56                       \\ \midrule
Captive       		& 133.91       & 180.79         & 46.88             & 33.33                      & 43.33                   & 10.00                       \\
\bottomrule
\end{tabular}
}
\caption{Overhead impact of CPU load 75\%}
\label{table:cpu75}
\end{table}

==> tables/cpu90.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lccc|ccc}
        \toprule

 \multirow{2}[2]{*}{ \textbf{SRT Category}}  & \multicolumn{3}{c}{\textbf{Overhead}} & \multicolumn{3}{c}{\textbf{Slow actions}} \\  \cmidrule{2-7}
& \textbf{CPU only}  & \textbf{CPU \& Monitoring}  & \textbf{$\Delta$} & \textbf{CPU only}  & \textbf{CPU \& Monitoring}  & \textbf{$\Delta$}\\   \midrule

Instantaneous 		& 15.39         & 20.36      & 4.98     & 83.64                           & 89.70                                  & 6.06                        \\ \midrule
Immediate     		& 26.21           & 41.89    & 15.68      & 31.67      & 50.00                                & 18.33                     \\ \midrule
Continuous Complex & 45.73  & 138.51        & 92.77         & 29.71                & 38.82                   & 9.12                                                     \\  \midrule
Continuous Simple  		& 116.36                & 183.63          & 67.27           & 52.22                            & 71.11                                   & 18.89                       \\  \midrule
Captive       	& 200.70      & 311.04      & 110.35          & 48.33                           & 58.33                             & 10.00                       \\ 
\bottomrule
\end{tabular}
}
\caption{Overhead impact of CPU load 90\%}
\label{table:cpu90}
\end{table}

==> tables/notepad.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lc|ccccccc}
        \toprule
%\multicolumn{2}{l|}{}                        & \multicolumn{6}{c}{With Monitoring}                                                                                                                                                                                 &                                                        
	 \begin{tabular}{c} \textbf{Action} \\ \textbf{Category} \end{tabular} 
	 & \textbf{Total}
	& \textbf{Instantaneous}
	& \textbf{Immediate}
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Simple} \end{tabular} 
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Complex} \end{tabular} 
	& \textbf{Captive}
	& $>$ \textbf{Captive}	
	& \begin{tabular}[c]{@{}c@{}} \textbf{Slow}\\\textbf{Actions [\%]}\end{tabular} \\ 
	 \midrule

Instantaneous   & 45    & \cellcolor{lightgray}40    & 0    &  \textbf{5}            & 0             & 0     & 0        &                                                 \textbf{11\%} \\ \midrule
Immediate       & 20    & 0     & \cellcolor{lightgray}19   &  \textbf{1}            & 0             & 0     & 0            &                                             \textbf{5\%} \\ \midrule
Continuous Simple    & 70    & 0     & 0    & \cellcolor{lightgray}48           & \textbf{6}             &  \textbf{11}    &  \textbf{5}     &                                                    \textbf{31\%} \\ \midrule
Continuous Complex   & 5     & 0     & 0    & 0            & \cellcolor{lightgray}5             & 0     & 0                             &                            \textbf{0\%} \\ \midrule
Captive         & 0     & 0     & 0    & 0            & 0             &  \cellcolor{lightgray}0     & 0                                               &          \textbf{0\%} \\
      \bottomrule
\end{tabular}
}
\caption{Notepad++: distribution of the typologies of actions with and without probe}
\label{notepadSA}
\end{table}

==> tables/overheadTable.tex <==
% !TEX root =  ../NIER_Extension.tex

% \begin{tabular}{lccc}
%         \toprule
% \textbf{Application}             & \textbf{Time Overhead {[}\%{]}}  & \textbf{RAM Overhead {[}\%{]}} & \textbf{Slow Actions {[}\%{]}} \\ \midrule
% Adobe Reader DC & 30.05                                      & 158.26            & 16.00                                                     \\ \midrule
% Notepad++               & 103.08                                      & 307.90             & 20.00                                                   \\ \midrule
% Paint.NET               & 34.35                                       & 115.22                   & 22.79                                             \\ \midrule
% VLC Media Player        & 16.49

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{l|ccccc|c}
\toprule
\textbf{Application} & \textbf{Instantaneous {[}\%{]}} & \textbf{Immediate {[}\%{]}} & \textbf{Continuous Simple {[}\%{]}} & \textbf{Continuous Complex {[}\%{]}} & \textbf{Captive {[}\%{]}} & \textbf{Overall Overhead {[}\%{]}}  \\ \midrule
Adobe Reader DC 	 & 		0.78	& 	-5.43	& 		49.22		& 		57.77		 & 		-   & 30.05 \\ \midrule
Notepad++            & 		8.09	& 	4.44	& 		198.67		& 		14.42		 & 		-   & 103.08 \\ \midrule
Paint.NET            & 		0.87	& 	83.15	& 		49.67		& 		35.68		 & 	18.62  & 34.35  \\ \midrule
VLC Media Player     & 		0.37	& 		-	& 		19.13		& 		21.59		 & 	-	   & 16.49  \\ 
 \midrule
 \textbf{Overall} 	 & 		2.72	& 	34.77	& 		69.00		& 		33.48		 & 	18.62  & 42.13  \\ 				
 \bottomrule
\end{tabular}
}

\caption{Overhead comparison between applications by system response time categories.}
\label{appComp}
\end{table}

==> tables/paint.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lc|ccccccc}
        \toprule
%\multicolumn{2}{l|}{}                        & \multicolumn{6}{c}{With Monitoring}                                                                                                                                                                                 &                                                        
	 \begin{tabular}{c} \textbf{Action} \\ \textbf{Category} \end{tabular} 
	 & \textbf{Total}
	& \textbf{Instantaneous}
	& \textbf{Immediate}
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Simple} \end{tabular} 
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Complex} \end{tabular} 
	& \textbf{Captive}
	& $>$ \textbf{Captive}	
	& \begin{tabular}[c]{@{}c@{}} \textbf{Slow}\\\textbf{Actions [\%]}\end{tabular} \\ 
	 \midrule
Instantaneous   & 35    & \cellcolor{lightgray}35    & 0    & 0            & 0             & 0       & 0  &  \textbf{0\%} \\ \midrule
Immediate       & 25    & 0     & \cellcolor{lightgray}0    & \textbf{24}           & 0             & \textbf{1}       & 0     &  \textbf{100\%} \\ \midrule
Continuous Simple    & 55    & 0     & 0    & \cellcolor{lightgray}45           & \textbf{7}             & \textbf{3}       & 0     &  \textbf{18\%}\\ \midrule
Continuous Complex   & 40    & 0     & 0    & 0            & \cellcolor{lightgray}29            & \textbf{11}      & 0   &  \textbf{28\%} \\ \midrule
Captive         & 60    & 0     & 0    & 0            & 0             & \cellcolor{lightgray}57      & \textbf{3}  & \textbf{5\%}    \\                           
      \bottomrule
\end{tabular}
}
\caption{Paint.NET: distribution of the typologies of actions with and without probe}
\label{paintSA}
\end{table}

==> tables/ram60.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lccc|ccc}
        \toprule

 \multirow{2}[2]{*}{ \textbf{SRT Category}}  & \multicolumn{3}{c}{\textbf{Overhead}} & \multicolumn{3}{c}{\textbf{Slow actions}} \\  \cmidrule{2-7}
& \textbf{RAM only}  & \textbf{RAM \& Monitoring}  & \textbf{$\Delta$} & \textbf{RAM only}  & \textbf{RAM \& Monitoring}  & \textbf{$\Delta$}\\   \midrule

%SRT Category  & RAM 60\% {[}\%{]} & Slow Actions {[}\%{]} & Monitoring {[}\%{]} & Slow Actions {[}\%{]} & $\Delta$ Overhead {[}\%{]} & $\Delta$ Slow Actions {[}\%{]} \\ \hline

Instantaneous & 0.61        & 3.88   & 3.27     & 0.61                             & 7.88                                 & 7.27                        \\ \midrule
Immediate     & 3.86       & 25.59     & 21.73      & 10.00                           & 41.67                              & 31.67                       \\ \midrule
Continuous Simple  & -1.42        & 71.50   & 72.98    & 1.47                           & 23.53                                 & 22.06                       \\ \midrule
Continuous Complex & -9.08        & 45.57     & 54.44     & 5.56                           & 24.44                           & 54.65                       \\ \midrule
Captive       & -2.96      & 20.72      & 23.68       & 1.67                          & 5.00                             & 3.33                        \\
\bottomrule
\end{tabular}
}
\caption{Overhead impact of RAM load 60\% with respect to the SRT Categories}
\label{table:ram60}
\end{table}

==> tables/ram75.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lccc|ccc}
        \toprule

 \multirow{2}[2]{*}{ \textbf{SRT Category}}  & \multicolumn{3}{c}{\textbf{Overhead}} & \multicolumn{3}{c}{\textbf{Slow actions}} \\  \cmidrule{2-7}
& \textbf{RAM only}  & \textbf{RAM \& Monitoring}  & \textbf{$\Delta$} & \textbf{RAM only}  & \textbf{RAM \& Monitoring}  & \textbf{$\Delta$}\\   \midrule
Instantaneous & 0.47      & 1.71    & 1.24     & 0.00                              & 4.84                                     & 4.84                        \\ \midrule
Immediate     & 0.98        & 25.05    & 24.07     & 6.67                               & 41.67                                   & 35.00                       \\  \midrule
Cont. Simple  & 1.35        & 71.85     & 70.51     & 2.94                               & 24.71                                  & 21.76                       \\  \midrule
Cont. Complex & 1.74       & 47.93     & 46.19    & 6.67                                & 26.67                                   & 20.00                       \\  \midrule
Captive       & 7.66       & 28.53   & 20.86         & 5.00                                & 6.67                                 & 1.67                        \\ 
\bottomrule
\end{tabular}
}
\caption{Overhead impact of RAM load 75\% with respect to the SRT Categories}
\label{table:ram75}
\end{table}

==> tables/ram90.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lccc|ccc}
        \toprule

 \multirow{2}[2]{*}{ \textbf{SRT Category}}  & \multicolumn{3}{c}{\textbf{Overhead}} & \multicolumn{3}{c}{\textbf{Slow actions}} \\  \cmidrule{2-7}
& \textbf{RAM only}  & \textbf{RAM \& Monitoring}  & \textbf{$\Delta$} & \textbf{RAM only}  & \textbf{RAM \& Monitoring}  & \textbf{$\Delta$}\\   \midrule

Instantaneous & 0.76         & 2.80    & 2.04      & 2.42                                 & 7.88                                  & 5.45                        \\  \midrule
Immediate     & 4.52      & 26.31     & 21.79         & 8.33                               & 41.67                                & 33.33                       \\  \midrule
Continuous Simple  & 7.04        & 73.05       & 66.01       & 3.82                            & 23.82                                 & 20.00                       \\  \midrule
Continuous Complex & 8.38     & 50.40        & 42.02        & 7.78                              & 32.22                                & 24.44                       \\  \midrule
Captive       & 9.46       & 30.89    & 21.43       & 3.33                               & 6.67                                   & 3.33                        \\
\bottomrule
\end{tabular}
}
\caption{Overhead impact of RAM load 90\% with respect to the SRT Categories}
\label{table:ram90}
\end{table}

==> tables/tableApplications.tex <==
% !TEX root =  ../NIER2017.tex
\begin{table}
\caption{Function calls rate, overhead, and slow actions.}\vspace{-0.3cm}
\label{overheadForFCallsRate}
\centering
\scriptsize
%\begin{adjustbox}{width=1\textwidth,keepaspectratio}
\begin{tabular}{|m{6em}|>{\centering}m{7em}|>{\centering}m{5em}|>{\centering\arraybackslash}m{6em}|}\hline

{\bf application} &  {\bf function calls rate (FCalls/s)} &  {\bf overhead (\%)} &  {\bf \slowactions (\%)} \\ \hline

Winzip		&	2,216 	&	23.7\%		&	7.14\%	\\ \hline
Paint.NET	& 	4,390	& 	48.4\%		&	12.09\%	\\ \hline
Acrobat DC	&	9,009	&	30.0\%		&	7.69\%	\\ \hline
VLC			&	21,663	&	41.9\%		&	7.14\%	\\ \hline
Notepad++	&	56,101	&	12.2\%		&	2.86\%	\\ \hline
MS Excel	&	2,977,154	&	387.9\%		&	51.95\%	\\ \hline
MS Outlook	&	3,029,380	&	269.4\%		&	48.05\%	\\ \hline

\end{tabular}
%\end{adjustbox}
%\vspace{-0.5cm}
\end{table}



==> tables/tableBuffer.tex <==
% !TEX root =  ../NIER_Extension.tex


\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{cccc}
        \toprule



%\begin{table}
%\caption{Effectiveness for different buffer sizes.} %\vspace{-0.3cm}
%\label{overheadForBuffer}
%\centering
%\scriptsize

%\begin{tabular}{|>{\centering}m{3em}|>{\centering}m{10em}|>{\centering}m{4em}|>{\centering\arraybackslash}m{7em}|}\hline

%{\bf buffer size (\textit{MB})} &  {\bf \slowactions \linebreak (\textit{num (\%)})} &  {\bf \ \linebreak overhead (\textit{\%})} &  {\bf RAM consumption \linebreak (\textit{MB})} \\ \hline
\textbf{Buffer size (MB)} & \textbf{\# Slow actions (\%)} & \textbf{Overhead (\%)} & \textbf{RAM consumption (MB)} \\ \midrule
0	&	20 		(18\%)		&	170\%	& 	192 \\ \midrule
1	& 	15	 	(13\%)		&	133\%	& 	198 \\  \midrule
25	&	16		(14\%)		&	104\%	&	243 \\  \midrule
50	&	17		(15\%)		&	97\%		&	281 \\  \midrule
75	&	21		(18\%)		&	128\%	&	321 \\  \midrule
100	&	16		(14\%)		&	108\%	&	355 \\  \midrule
200	&	16		(14\%)		&	93\%		&	485 \\ 

\bottomrule
\end{tabular}
}
\caption{Effectiveness for different buffer sizes.} %\vspace{-0.3cm}
\label{overheadForBuffer}
\end{table}


==> tables/vlc.tex <==
% !TEX root =  ../NIER_Extension.tex

\begin{table}[h]
\resizebox{\textwidth}{!}{%
  \centering
\begin{tabular}{lc|ccccccc}
        \toprule
%\multicolumn{2}{l|}{}                        & \multicolumn{6}{c}{With Monitoring}                                                                                                                                                                                 &                                                        
	 \begin{tabular}{c} \textbf{Action} \\ \textbf{Category} \end{tabular} 
	 & \textbf{Total}
	& \textbf{Instantaneous}
	& \textbf{Immediate}
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Simple} \end{tabular} 
	& \begin{tabular}{c} \textbf{Continuous} \\ \textbf{Complex} \end{tabular} 
	& \textbf{Captive}
	& $>$ \textbf{Captive}	
	& \begin{tabular}[c]{@{}c@{}} \textbf{Slow}\\\textbf{Actions [\%]}\end{tabular} \\ 
	 \midrule
Instantaneous   & 30    &  \cellcolor{lightgray}30    & 0    & 0            & 0             & 0     & 0                                                         & \textbf{0\%}                                                      \\   \midrule
Immediate       & 0     & 0     &  \cellcolor{lightgray}0    & 0            & 0             & 0     & 0                                                         & \textbf{0\%}                                                      \\   \midrule
Cont. Simple    & 125   & 0     & 0    &  \cellcolor{lightgray}99           &  \textbf{26}            & 0     & 0                                                         & \textbf{21\%}                                                      \\   \midrule
Cont. Complex   & 30    & 0     & 0    & 0            &  \cellcolor{lightgray}24            &  \textbf{6}     & 0                                                         &\textbf{20\%}                                                      \\   \midrule
Captive         & 0     & 0     & 0    & 0            & 0             &  \cellcolor{lightgray}0     & 0                                                         & \textbf{0\%}                                                      \\   \bottomrule
\end{tabular}
}
\caption{VLC Media Player: distribution of the typologies of actions with and without probe}
\label{vlcSA}
\end{table}
